Convergence of the height process of supercritical Galton-Watson forests with an application to the configuration model in the critical window

We show joint convergence of the Lukasiewicz path and height process for slightly supercritical Galton-Watson forests. This shows that the height processes for supercritical continuous state branching processes as constructed by Lambert (2002) are the limit under rescaling of their discrete counterparts. Unlike for (sub-)critical Galton-Watson forests, the height process does not encode the entire metric structure of a supercritical Galton-Watson forest. We demonstrate that this result is nonetheless useful, by applying it to the configuration model with an i.i.d. power-law degree sequence in the critical window, of which we obtain the metric space scaling limit in the product Gromov-Hausdorff-Prokhorov topology, which is of independent interest.

==> Percolation.tex <==
 \subsubsection{Relation to percolation}\label{subsec.percolation}
We will illustrate that the law of a degree sequence that is obtained by bond percolation on the half-edges of an i.i.d.\ degree sequence in the supercritical regime satisfies the conditions of Theorem \ref{thm.convgraphscriticalwindow}. \\
Let $D$ be a random variable in $\N$ that satisfies $\E [D]=\mu$, $\E [D^2]=\rho>2\mu$ and $\P (D=k)\sim ck^{-(\alpha+2)}$ for $\alpha \in (1,2)$ as $k\rightarrow \infty$. Define $C_{\alpha}=\frac{c\Gamma(2-\alpha)}{\alpha(\alpha-1)}$, so that the Laplace transform $\cL_D$ of $D$ satisfies
$$\cL_D(\theta)=\E [\exp (-\theta D)]=1-\mu \theta +\frac{\rho}{2}\theta^2-\frac{C_{\alpha}}{\alpha+1} \theta^{\alpha+1}+o(\theta^{\alpha+1})$$ for $\theta \rightarrow 0$. View $D$ as the degree distribution. Then, keep every half-edge with probability 
$$p(\lambda,n)=\frac{1+\lambda n^{-{(\alpha-1)/(\alpha+1)}}}{\frac{\rho}{\mu}-1},$$ and call the resulting degree distribution $B^{(\lambda,n)}$. We will check the conditions of Theorem \ref{thm.convgraphscriticalwindow} for $B^{(\lambda,n)}$. \\
Then, note that the Laplace transform $\cL_{B^{(\lambda,n)}}$ of $B^{(\lambda,n)}$ satisfies 
\begin{equation}\label{eq.laplacebinomial}
        \cL_{B^{(\lambda,n)}}(\theta)=\E [\exp(D\log ( 1-p(\lambda,n)+p(\lambda,n)e^{-\theta}))],
\end{equation}
such that
 \begin{align*}
     \cL_{B^{(\lambda,n)}}(\theta)
    &=1-p(\lambda,n)\mu\theta+p(\lambda,n)\mu\left(2+\lambda n^{-{(\alpha-1)/(\alpha+1)}}\right)\frac{\theta^2}{2}-\frac{C_{\alpha}}{\alpha+1}p(\lambda,n)^{\alpha+1}\theta^{\alpha+1}+o(\theta^{\alpha+1}) 
\end{align*}
as $\theta\to 0$. This implies that conditions \ref{cond1}, \ref{cond2} and \ref{cond3} are satisfied with $\mu_n=p(\lambda,n)\mu\to\mu/(\frac{\rho}{\mu}-1)$ and  $c_n=cp(\lambda,n)^{\alpha+1}\to c/(\frac{\rho}{\mu}-1)$ as $n\to \infty$. \\
We now check condition \ref{cond3}. We will drop the dependency on $\lambda$ from the notation, unless necessary to avoid confusion. Let $\tilde{D}$ be a random variable with the size-biased law of $D$, i.e.\ for all $k\in \N$, $$\P(\tilde{D}=k)=\frac{k\P(D=k)}{\E[D]},$$ and similarly, let $\tilde{B}_n$ be a random variable with the size-biased law of ${B}^{(n,\lambda)}$, i.e.\  $$\P(\tilde{B}_n=k)=\frac{k\P({B}^{(n,\lambda)}=k)}{\E\left[{B}^{(n,\lambda)}\right].$$
Let $g_{{\tilde{D}}-1}(x)$ and $g_{{\tilde{B}}_n-1}(x)$ be the probability generating function of $\tilde{D}-1$ and $\tilde{B}}_n-1$ respectively, such that \eqref{eq.laplacebinomial} implies that
$$g_{{\tilde{B}}_n-1}(x)=g_{\tilde{D}-1}\left(1-p(\lambda,n)+p(\lambda,n)x\right).$$
Note that, for $g_{{\tilde{B}}_n-1}^{\circ k }$ the $k^{th}$ iterate of $g_{{\tilde{B}}_n-1}$, condition \ref{cond4} is equivalent to
\begin{equation}\label{eq.treesdie}\liminf_{n\to\infty}\left(g_{{\tilde{B}}_n-1}^{\circ \lfloor \delta n^{(\alpha-1)/(\alpha+1)}\rfloor }(0)\right)^{\lfloor n^{1/(\alpha+1)}\rfloor}>0.\end{equation}
By the proof of Proposition 5.25 in \cite{broutinLimitsMultiplicativeInhomogeneous2020}, it sufficient if we show that, for $t\in (0,\infty)$, and $r_n(t)$ the value such that
$$\int_{r_n(t)}^1 \frac{dr}{g_{{\tilde{B}}_n-1}(1-r)-1+r}=n^{(\alpha-1)}{(\alpha+1)}t,$$
we have that
$$\limsup_{n\to\infty}n^{1/(\alpha+1)}r_n(t)<\infty.$$
Note that 
\begin{align*}
    \int_{r_n(t)}^1 \frac{dr}{g_{{\tilde{B}}_n-1}(1-r)-1+r}&=\int_{r_n(t)}^1 \frac{dr}{g_{\tilde{D}-1}\left(1-p(\lambda,n)r\right)-1+r}\\
    \int_{p(\lambda,n)r_n(t)}^{p(\lambda,n)} \frac{ds}{p(\lambda,n)g_{\tilde{D}-1}\left(1-s\right)-p(\lambda,n)+s}
\end{align*}
Elementary calculation yields that 
$$g_{\tilde{D}-1}\left(1-s\right)=1-\left(\rho/\mu-1)s+\frac{C_\alpha}{\mu}s^\alpha+o(s^\alpha)$$ 
as $s\to \infty$, which implies that
$$p(\lambda,n)g_{\tilde{D}-1}\left(1-s\right)-p(\lambda,n)+s=-\lambda n^{-(\alpha-1)/(\alpha+1)}s+p(\lambda,n)\frac{C_\alpha}{\mu}s^\alpha+p(\lambda,n)o(s^\alpha).$$






% We will give a heuristic argument for how the family of degree distributions defined above can be related to bond percolation on a supercritical random graph with i.i.d.\ power-law degrees. \\
% Suppose that we have degrees distributed as $D$, satisfying $\P (D=k)\sim ck^{-(\alpha+2)}$ for $\alpha \in (1,2)$ as $k\rightarrow \infty$, with $\E [D^2]=\rho$ and $\E [D]=\mu$, so that $$\cL_D(\theta)=\E [\exp (-\theta D)]=1-\mu \theta +\frac{\rho}{2}\theta^2-\frac{C_{\alpha}}{\alpha+1} \theta^{\alpha+1}+o(\theta^{\alpha+1})$$ for $\theta \rightarrow 0$ and for $C_{\alpha}=\frac{c\Gamma(2-\alpha)}{\alpha(\alpha-1)}$. Let $Z$ be distributed as $\P(Z=k)=\frac{k\P(D=k)}{\E[D]}$. As will later be motivated, we want $Z-1$ to have mean larger than $1$ for the random graph to be supercritical, so we require $\rho>2\mu$.  Conditionally on $D$, for $p\in (0,1)$, let $B^{(p)}\sim \operatorname{Bin}(D,p)$. This is approximately the degree distribution after bond percolation at parameter $p$ on a random graph with i.i.d.\ degrees distributed as $D$, although we ignore dependence between the degrees of different vertices. This can be dealt with using an argument like introduced by Janson in \cite{Janson2009a}, but this will be omitted in the heuristic argument presented here.  We claim that one way to realise a family of degree distributions in the critical window is to take them distributed as $B^{(p)}$ for a family of values of $p$. Let $I_1,I_2,\dots$ be i.i.d.\ random variables with $\operatorname{Ber}(p)$ distribution.
% Note that  
% \begin{align*}
% \cL_B(\theta)=\E[\exp(-\theta B^{(p)})]&= \E\left[\exp\left(-\theta \sum\limits_{i=1}^D I_i\right)\right]\\
% &=\E [\exp(D\log ( 1-p+pe^{-\theta}))]\\
% &=1+\mu\left(-p\theta+\frac{p}{2}\theta^2-\frac{p^2}{2}\theta^2\right) + \frac{\rho}{2}p^2\theta^2 -\frac{C_{\alpha}}{\alpha+1}p^{\alpha+1}\theta^{\alpha+1}+o(\theta^{\alpha+1})\\
% &=1-p\mu\theta+\frac{1}{2}(p\mu-p^2\mu+p^2\rho)\theta^2 -\frac{C_{\alpha}}{\alpha+1}p^{\alpha+1}\theta^{\alpha+1}+o(\theta^{\alpha+1})
% \end{align*}
%  Hence, up to the terms of order $\alpha+1$, the Laplace transform of $B^{(p)}$ around $0$ corresponds to the Laplace transform of a random variable $D^{(p)}$ with power law behaviour such that $\E[D^{(p)}]=p\mu$, $\E[(D^{(p)})^2]=p\mu-p^2\mu+p^2\rho$ and $\P(D^{(p)}=k)\sim cp^{\alpha+1} k^{-(\alpha+2)}$. Set $$p=p(\lambda,n)=\frac{1+\lambda n^{-{(\alpha-1)/(\alpha+1)}}}{\frac{\rho}{\mu}-1}=\frac{1+\lambda n^{-{(\alpha-1)/(\alpha+1)}}}{\E[Z-1]}.$$ Then, for $Z^{(p)}$ a random variable with the size-biased distribution of $D^{(p)}$, we have that 
% \begin{enumerate}
% \item $\E[D^{(p)}]=\frac{1+\lambda n^{-{(\alpha-1)/(\alpha+1)}}}{\E[Z^{(p)}-1]}\mu\to \frac{\mu}{\E[Z^{(p)}-1]}$ as $n\to\infty$,
%     \item ${\E[(D^{(p)})^2]}=\left(2+\lambda n^{-{(\alpha-1)/(\alpha+1)}}\right){\E[D^{(p)}]}$,
%     \item $\P(D^{(p)}=k)\sim c\left(\frac{1+\lambda n^{-{(\alpha-1)/(\alpha+1)}}}{\E[Z^{(p)}-1]}\right)^{\alpha+1}k^{-(\alpha+2)}$ as $k\to \infty$ with $c\left(\frac{1+\lambda n^{-{(\alpha-1)/(\alpha+1)}}}{\E[Z^{(p)}-1]}\right)^{\alpha+1}\to \frac{c}{\E[Z^{(p)}-1]^{\alpha+1}}$ as $n\to\infty$
% \end{enumerate}
% as desired. This suggests that the chosen definition of the critical window can indeed be linked to percolation. \\
